Towards Multi-Task Multi-Modal Models: A Video Generative Perspective

Advancements in language foundation models have primarily fueled the recent surge in artificial intelligence. In contrast, generative learning of non-textual modalities, especially videos, significantly trails behind language modeling. This thesis chronicles our endeavor to build multi-task models for generating videos and other modalities under diverse conditions, as well as for understanding and compression applications. Given the high dimensionality of visual data, we pursue concise and accurate latent representations. Our video-native spatial-temporal tokenizers preserve high fidelity. We unveil a novel approach to mapping bidirectionally between visual observation and interpretable lexical terms. Furthermore, our scalable visual token representation proves beneficial across generation, compression, and understanding tasks. This achievement marks the first instances of language models surpassing diffusion models in visual synthesis and a video tokenizer outperforming industry-standard codecs. Within these multi-modal latent spaces, we study the design of multi-task generative models. Our masked multi-task transformer excels at the quality, efficiency, and flexibility of video generation. We enable a frozen language model, trained solely on text, to generate visual content. Finally, we build a scalable generative multi-modal transformer trained from scratch, enabling the generation of videos containing high-fidelity motion with the corresponding audio given diverse conditions. Throughout the course, we have shown the effectiveness of integrating multiple tasks, crafting high-fidelity latent representation, and generating multiple modalities. This work suggests intriguing potential for future exploration in generating non-textual data and enabling real-time, interactive experiences across various media forms.

==> overviews/impact.tex <==
\paragraph{Impact in Academia}

\paragraph{Impact in Industry}

\paragraph{Social Impacts}

\paragraph{Media Coverage}

==> overviews/lq.tex <==
While showing promising outcomes, the techniques introduced in \cref{chap:3dvq,chap:spae} encounter challenges in recuperating intricate textual elements such as written text and human facial features. An inherent limitation lies in the vector quantizer module, which struggles to scale effectively with expanding vocabulary sizes.
Addressing this, the forthcoming \cref{chap:magvitv2} adopts scalar quantization, drawing inspiration from the realm of video compression. This new approach brings forth numerous architectural advancements aimed at enhancing the restoration of nuanced visual details. Moreover, it facilitates a unified tokenization method for images and videos, which encompass causal interdependencies. Importantly, this framework establishes a cohesive foundation for tasks spanning generation, compression, and comprehension, yielding an unprecedented multi-purpose representation.
The overarching goal of this effort is to propel the dimensions of quality, spatial-temporal expansiveness, and task flexibility inherent to discrete visual representations to new heights.


==> overviews/magbit.tex <==
We propose to use a single transformer model to tackle \emph{compression, generation, and understanding} tasks involving the aforementioned modalities.
Leveraging the unified token representation from \cref{chap:magvitv2}, the latent generative transformer operates in the joint feature space of the tokenizer, which is closely connected to the raw pixels but much more compact.
We introduce new techniques for more effective modeling of the large and dimension-independent vocabulary, leveraging its natural form of binary variables.
As a result, we show strong performance on all three types of tasks for both images and videos using a single model. 


==> papers/argus/sections/abs.tex <==
Activity detection is one of the attractive computer vision tasks to exploit the video streams captured by widely installed cameras.
Although achieving impressive performance, conventional activity detection algorithms are usually designed under certain constraints, such as using trimmed and/or object-centered video clips as inputs.
Therefore, they failed to deal with the multi-scale multi-instance cases in real-world unconstrained video streams, which are untrimmed and have large field-of-views.
Real-time requirements for streaming analysis also mark brute force expansion of them unfeasible.

To overcome these issues, we propose \textit{Argus++}, a robust real-time \emph{multi-task} activity detection system for analyzing unconstrained video streams. 
The design of \textit{Argus++} introduces \textit{overlapping spatial-temporal cubes} as an intermediate concept of activity proposals to ensure coverage and completeness of activity detection through over-sampling.
The overall system is optimized for real-time processing on standalone consumer-level hardware.
Extensive experiments on different surveillance and driving scenarios demonstrated its superior performance in a series of activity detection benchmarks, including CVPR ActivityNet ActEV 2021, NIST ActEV SDL UF/KF, TRECVID ActEV 2020/2021, and ICCV ROAD 2021.

% We propose an action recognition system for surveillance scenarios, which wins TRECVID 2020~\cite{2020trecvidawad} Activities in Extended Video (ActEV\footnote{\url{https://actev.nist.gov}}) Challenge with a large advantage of 23.8\%~\cite{yucmu} ahead the runner up system. 
% Our system develops a dense spatial-temporal proposal generation model which collaborates with the state-of-the-art action classifiers. The proposed system utilizes multiple state-of-the-art modules and is trained on VIRAT Dataset with only released annotations. In this paper, we demonstrate the architecture and algorithms with technique details of the winner system.


==> papers/documentnet/sections/abstract.tex <==
Document understanding tasks, in particular, Visually-rich Document Entity Retrieval (\taskname{}), have gained significant attention in recent years thanks to their broad applications in enterprise AI.
However, publicly available data have been scarce for these tasks due to strict privacy constraints and high annotation costs.
% as document images often contain personally identifiable information, publicly available data have been scarce, not only because of privacy constraints but also the costs of acquiring annotations.
To make things worse, the non-overlapping entity spaces from different datasets hinder the knowledge transfer between document types.
In this chapter, we propose a method to collect massive-scale and weakly labeled data from the web to benefit the training of \taskname{} models. 
% Such a method will generate a huge amount of document image data to compensate for the lack of training data in many VDER settings. Moreover, 
The collected dataset, named \dataname{}, does not depend on specific document types or entity sets, making it universally applicable to all \taskname{} tasks.
The current \dataname{} consists of 30M documents spanning nearly 400 document types organized in a four-level ontology.
Empowered by \dataname{}, we present a lightweight multimodal architecture named \modelname{}, which can learn a unified representation from text, layout, and image crops without needing extra visual pretraining.
Experiments on a set of broadly adopted VDER tasks show significant improvements when \dataname{} is incorporated into the pre-training.
%  for both classic and few-shot learning settings.
With the recent emergence of large language models (LLMs), \dataname{} provides a large data source to extend their multimodal capabilities for VDER.
% as VDER tasks are increasingly being studied by large language models (LLM), we believe that such a dataset can potentially benefit the training of LLMs especially those with multimodal capabilities.


==> papers/documentnet/sections/antology.tex <==
\subsection{Financial Documents}

\begin{itemize}[nosep]
\item accounts receivable aging report
\item bill of exchange pdf
\item invoice
\item receipt
\item loan estimate
\item loan application form
\item credit report pdf
\item employee insurance enrollment form
\item property insurance declaration page
\item renters insurance addendum
\item auto insurance card
\item dental insurance card
\item dental insurance verification form
\item vision insurance card
\item medical insurance card
\item liability insurance certificate
\item insurance cancellation letter
\item life insurance application form
\item flood elevation certificate
\item flood insurance application form
\item hazard insurance application form
\item tax return form
\item form 1040 schedule C
\item form 1040 schedule E
\item form 1040 schedule D
\item form 1040 schedule B
\item form 1040 nr
\item form 1040 sr
\item form 4506T EZ
\item form 4506T
\item form 4506 C
\item transfer of residence form 1076
\item property tax bill
\item W2
\item W4
\item 1099 B
\item 1099-MISC
\item 1099-NEC
\item 1099 DIV
\item 1099 G PDF
\item 1099 R
\item 1099 INT
\item SSA 1099 form
\item 1120 form
\item 1120S Form
\item form 1065
\item W7 form
\item W8BEN form
\item W9 form
\item SS4 form
\item form 940 pdf
\item form 5498
\item ucc 1 form
\item bank statement
\item personal check
\item check deposit slip pdf
\item credit union statement pdf
\item credit card authorization form
\item credit card
\item debit card
\item credit card statement
\item TSP election form
\item 401k enrollment form
\item IRA distribution request form
\item stock certificate
\item stock purchase agreement
\item bond certificate
\item bond purchase agreement
\item mutual fund consolidated account statement
\item HSA enrollment form
\item FSA enrollment form
\item verification of employment pdf
\item wage paystub
\item income verification letter
\item music recording contract
\item food stamp application form
\item us treasury check
\item child welfare services application form
\item medicaid card
\item medicaid application form
\item club application
\item membership renewal letter pdf
\item mortgage statement
\item rent invoice
\item electric bill
\item pg\&e care fera application pdf
\item gas bill
\item water bill
\item waste management invoice
\item spectrum internet bill pdf
\item phone bill pdf
\item car payment agreement
\item student loan payment agreement
\item child support agreement
\item child support receipt
\item elder care facility agreement
\item debt paymen tletter
\item demand for payment letter
\item magazine subscription form
\item streaming service agreement
\item gym waiver form
\item gym membership cancellation letter
\item gym membership card
\item massage therapy waiver
\item HOA agreement
\item HOA dues letter
\item urla form 1003
\item home appraisal report
\item security instrument
\item ucdp summary report
\item audit findings report pdf
\item sales contract
\item purchase agreement
\item title commitment pdf
\item earnest money deposit pdf
\item patriot act disclosure
\item owner occupancy affidavit form
\item compliance agreement
\item name affadavit
\item notice of right to reclaim abandoned property
\item VBA 26-0551 debt questionnaire pdf
\item VBA 26-8923 form pdf
\item USDA-AD 3030
\item loan application pdf
\item homeowner insurance declaration page
\item 1040
\item wage and tax statement
\item employee's withholding certificate
\item miscellaneous income form
\item nonemployee compensation form
\item dividends and distributions form
\item certain government payments
\item distributions from pensions
\item social security benefits form
\item form 1005
\item stimulus check pdf
\item waste management bill
\item comcast internet bill pdf
\item car loan payment agreement
\item gym release form
\item one and the same person affadavit
\item xfinity internet bill pdf
\item car payment contract
\end{itemize}

\subsection{Legal Documents}

\begin{itemize}[nosep]
\item birth certificate
\item social security card
\item social security form
\item ssa 89 form
\item social security change in information form
\item passport book
\item passport card
\item new passport application
\item passport renewal application
\item green card
\item green card application form
\item naturalization certificate
\item N-400 form pdf
\item living will sample
\item living will form
\item living will declaration
\item voter identification card
\item disability card
\item death certificate
\item death certificate application
\item name change form
\item state issued identification card
\item prenup form
\item postnuptial agreement
\item marriage license
\item marriage certificate
\item application for marriage license
\item family court cover sheet
\item complaint for divorce no children
\item complaint for divorce with children
\item divorce summons
\item divorce certificate
\item domestic partnership application form
\item domestic partnership certificate
\item domestic partnership termination form
\item separation agreement
\item pet custody agreement form 
\item pet ownership transfer form
\item child adoption certificate
\item child power of attorney
\item child visitation form
\item daycare contract
\item child custody agreement
\item child support modification form
\item free minor travel consent form
\item child identity card
\item DNA paternity test order form
\item petition for declaration of emancipation of minor
\item vehicle registration card
\item vehicle registration form
\item vehicle registration renewal notice
\item vehicle certificate of title
\item motor vehicle transfer form
\item driver's license
\item application for driver's license
\item truck driver application
\item learner's permit card
\item pilot's license card
\item vehicle leasing agreement
\item motor vehicle power of attorney
\item mortgage interest credit form
\item mortgage application form
\item mortgage verification form
\item mortgage loan modification form
\item real estate deed of trust
\item mortgage deed
\item warranty deed
\item quitclaim deed
\item usps mail forwarding form PDF
\item property power of attorney
\item notice of intent to foreclose
\item closing disclosure
\item HUD 92541 form
\item HUD 54114 form
\item HUD 92561 form
\item FHA loan underwriting and transmittal summary
\item form HUD92051
\item form HUD 92900-A
\item form HUD 92544
\item form HUD 92900 B important notice to housebuyers
\item form HUD 92900 WS mortgage credit analysis worksheet
\item Form HUD 92800 Conditional Commitment
\item SFHDF
\item lease agreement
\item lease application
\item notice to enter
\item notice of intent to vacate premises
\item notice of lease violation
\item pay rent or quit
\item lease offer letter
\item roommate agreement
\item eviction notice form
\item lease termination letter
\item lease renewal agreement
\item pet addendum
\item notice of rent increase
\item sublease agreement
\item record of immunization
\item allergy record sheet
\item allergy immunotherapy record
\item medication log
\item prescription sheet
\item disability documentation
\item advance directive form
\item DNA test request form
\item medical power of attorney
\item health care proxy form
\item revocation of power of attorney
\item dnr form
\item hipaa release form
\item hipaa complaint form
\item health history form
\item birth plan form
\item new patient form
\item child medical consent
\item grandparent medical consent for minor
\item medical treatment authorization form
\item dental policy and procedure document
\item endodontic treatment consent form
\item denture treatment consent form
\item dental patient referral form
\item patient dismissal letter
\item dental record release form
\item oral surgery postop instructions
\item refusal of dental treatment form
\item tooth extraction consent form
\item corrective lens prescription pdf
\item military id card
\item dd214
\item honorable discharge certificate
\item supreme court distribution schedule pdf
\item case docket pdf
\item jury summons pdf
\item jury duty excuse letter
\item supplemental juror information pdf
\item attorney termination letter
\item certificate of good standing
\item attorney oath of admission pdf
\item substitution of attorney
\item notice of appearance of counsel
\item bankruptcy declaration form
\item notice of lawsuit letter
\item court summons pdf
\item arrest warrant pdf
\item promissory note
\item tolling agreement pdf
\item notary acknowledgement form
\item cease and desist letter
\item condominium rider pdf
\item adjustable rate rider pdf
\item family rider form 1-4 pdf
\item balloon rider form pdf
\item second home rider pdf
\item revocable trust rider form pdf
\item pud rider pdf
\item birth certificate form
\item ssn card
\item application for a social security card
\item application for naturalization pdf
\item legal name change form
\item state issued ID
\item prenup sample
\item postnuptial agreement sample
\item declaration of domestic partnership
\item marriage separation agreement
\item minor power of attorney
\item request for child custody form
\item child care contract
\item motion to adjust child support
\item child travel consent form
\item vehicle registration application
\item vehicle certificate of title
\item driver's license application
\item mortgage loan application form
\item real estate power of attorney
\item foreclosure letter notice
\item rental agreement
\item rental application
\item landlord notice to enter
\item intent to vacate rental
\item notice to pay rent or quit
\item roommate contract
\item eviction notice pdf
\item early lease termination letter
\item pet addendum to lease agreement
\item rent increase letter
\item vaccine record form
\item prescription sample
\item healthcare directive form
\item do not resuscitate form
\item medical records release form
\item medical history form
\item new patient registration form
\item child medical release form
\item root canal consent form
\item eyeglasses prescription pdf
\item military discharge form
\item notice of intent to sue
\item ssn application
\item name change form example
\item prenuptial agreement sample
\item marital separation form
\item motion to modify child support
\item tenant application
\item notice to enter premises
\item notice to vacate
\item notice to quit
\item notice of lease termination
\item doctor prescription
\item patient history form
\item patient intake form
\item consent to treat minor
\item form petition for name change
\item medical intake form
\end{itemize}

\subsection{Business Documents}

\begin{itemize}[nosep]
\item articles of incorporation
\item corporate bylaws
\item operating agreement
\item shareholder agreement
\item memorandum of understanding
\item expense report
\item purchase of business agreement
\item purchase order
\item invoice pdf
\item late payment reminder letter
\item arbitration agreement pdf
\item business contract
\item payment agreement document
\item end user license agreement
\item licensing agreement pdf
\item job application form
\item employment offer letter
\item employment rejection letter
\item employment agreement
\item resume
\item employment resignation letter
\item notice of contract termination
\item notice of employmen termination
\item nda pdf
\item non compete agreement
\item leave of absence request
\item employment evaluation form
\item overdue payment reminder letter
\item job application pdf
\item job offer letter
\item job rejection letter
\item employment contract
\item contract termination letter
\item non disclosure agreement
\end{itemize}

\subsection{Education Documents}

\begin{itemize}[nosep]
\item research papers pdf
\item certificate of enrollment
\item high school transcript
\item high school diploma
\item college diploma
\item college transcript
\end{itemize}


==> papers/documentnet/sections/limitations.tex <==
EMNLP 2023 requires all submissions to have a section titled ``Limitations'', for discussing the limitations of the paper as a complement to the discussion of strengths in the main text. This section should occur after the conclusion, but before the references. It will not count towards the page limit.  

The discussion of limitations is mandatory. Papers without a limitation section will be desk-rejected without review.
ARR-reviewed papers that did not include ``Limitations'' section in their prior submission, should submit a PDF with such a section together with their EMNLP 2023 submission.

While we are open to different types of limitations, just mentioning that a set of results have been shown for English only probably does not reflect what we expect. 
Mentioning that the method works mostly for languages with limited morphology, like English, is a much better alternative.
In addition, limitations such as low scalability to long text, the requirement of large GPU resources, or other things that inspire crucial further investigation are welcome.


==> papers/documentnet/sections/model.tex <==
% None of the existing pre-trained document models can fully make use of the modalities available in \dataname{}.
To take advantage of all the modalities available in \dataname{},
% To leverage the collected data for document pre-training, 
we build a lightweight transformer model named \modelname{} for document pre-training.
% to take advantage of all the modalities in the dataset.
Table \ref{tab:pretrain} lists the pre-training objectives and corresponding target modalities.
% \modelname{} is pre-trained with the objectives listed in Table \ref{tab:pre-train}.

\modelname{} is built upon the BERT~\cite{devlin2019bert} architecture similar to LayoutLM~\cite{xu2020layoutlm} and LayoutLMv2~\cite{xu2021layoutlmv2}.
Figure \ref{fig:pretrain_arch} illustrates the pre-training pipeline.
We highlight the new designs for multimodal pretraining here and defer more details into App. \ref{app:model}.

\input{papers/documentnet/tables/pretrain}
\input{papers/documentnet/tables/ablation}
% \vspace{-2mm}
\paragraph{Multimodal tokenization and embedding.}
With a pre-defined text tokenizer, \eg WordPiece~\cite{wu2016google}, we first tokenize the OCR characters into a sequence of text tokens $\rvc$.
% $\rvp$ represents the 1D position of the tokens ranging from $0$ to $|\rvc|-1$.
For each token $\ervc_i$, we obtain its bounding box $\ervb_i = (x_0, y_0, x_1, y_1)_i$ by taking the union of the bounding boxes of its characters.
We enlarge the bounding box by a context ratio $r$ on each side and obtain the corresponding visual image crop $\ervv_i$ for each token from the raw image.
To model visual information, we add a crop embedding by linearly projecting the flattened pixels in the image crop, following ViT~\cite{dosovitskiy2020image}.

% \vspace{-2mm}
\paragraph{Masked crop modeling.}
In addition to predicting the text token in the MMLM objective,
A \modelname{} parameterized by $\theta$ also predicts the visual modality by reconstructing the image crops for the masked tokens, in a way similar to MAE~\cite{he2022masked}.
It is formulated as a regression problem with a linear layer outputing flattened pixels and the objective is
% \vspace{-2mm}
\begin{equation}
    \Ls_\mathit{MCM} = \mathop{\E}_{\text{data}} \Big[ \sum_{\ervc_i \in \gM} \left\|{f_\theta(\overline{\rvc}, \overline{\rvv}, \rho)}_i - \ervv_i\right\|_2^2 \Big]
\end{equation}
where $\overline{\rvc}$ and $\overline{\rvv}$ denotes the masked tokens and crops according to mask $\gM$.
$\rho$ is the position and layout embeddings.

% \vspace{-2mm}
\paragraph{Token tagging.}
With fully unmasked sequences, \modelname{} is pre-trained to predict the token tags $\rvt$ with a separate head.
% The tags are extracted from an external text tagger as described in Section \ref{sec:ocr}.
Since each token may have multiple tags, it is formulated as a multi-label classification problem with binary cross-entropy losses.
% as 
% % \vspace{-2mm}
% \begin{equation}
% \Ls_\mathit{TT} = \mathop{\E}_{\text{data}} \text{BCE}\Big[g_\theta (\rvc, \rvv, \rho)_{i, k} \mid \ervt_{i, k}\Big]
% % \begin{aligned}
% %   \Ls_\mathit{TT} &= \mathop{\E} \Big[ \sum_{i, k} -\ervt_{i, k} \log p_\theta (\ervt_{i, k} \mid [\rvc, \rvv, \rho]) \\
% %   &-(1 - \ervt_{i, k}) \log (1 -  p_\theta (\ervt_{i, k} \mid [\rvc, \rvv, \rho])))  \Big]
% % \end{aligned}
% \end{equation}
% where $k=1,2,\cdots,K$ refers to the $K$ types of tags.


==> papers/documentnet/tables/few-shot.tex <==
\begin{table*}[tp]
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ll | ccc |ccc |ccc}

% \toprule
%  Settings & Model  & \multicolumn{3}{c}{\makecell{IIT-CDIP subset (11M)}}     & \multicolumn{3}{c}{\makecell[l]{IIT-CDIP subset (11M)\\\ \ + \dataname-v1 (9.9M)}} & \multicolumn{3}{c}{\makecell[l]{IIT-CDIP subset (11M)\\\ \ + \dataname-v2 (30M)}} \\
% \midrule
% % The Original Model on 100  Few-shot Tasks 4-way 2-shot
% 4-way 2-shot & \modelname
% & 0.099& 0.253& 0.062 & 0.102& 0.217 & 0.067  &\textbf{0.133}&\textbf{0.263}&\textbf{0.090}\\
% 4-way 2-shot & \modelname + Hier 
% & 0.108& 0.103& 0.114 & 0.121 & 0.114 &  0.132  &\textbf{0.147}&\textbf{0.137}&\textbf{0.160}\\
% 4-way 4-shot & \modelname + Hier 
% & 0.115 & 0.110 & 0.123 & 0.129& 0.125 & 0.134   &\textbf{0.157}&\textbf{0.155}&\textbf{0.160}\\
% \bottomrule
\toprule
 Datasets & \makecell[r]{Setting\\Prediction Head}  &   \multicolumn{3}{c}{\makecell{4-way 2-shot\\Simple}}    & \multicolumn{3}{c}{\makecell{4-way 2-shot\\Hierarchical}} & \multicolumn{3}{c}{\makecell{4-way 4-shot\\Hierarchical}} \\
\midrule
& & F1 & Prec. & Recall & F1 & Prec. & Recall & F1 & Prec. & Recall \\
\multicolumn{2}{l|}{IIT-CDIP} & 0.099& 0.253& 0.062 &0.108& 0.103& 0.114 & 0.115 & 0.110 & 0.123 \\
\multicolumn{2}{l|}{IIT-CDIP + \emph{\dataname-v1}} & 0.102& 0.217 & 0.067  &0.121 & 0.114 &  0.132  &0.129& 0.125 & 0.134\\
\multicolumn{2}{l|}{IIT-CDIP + \emph{\dataname-v2}} &  \textbf{0.133}&\textbf{0.263}&\textbf{0.090} & \textbf{0.147}&\textbf{0.137}&\textbf{0.160} & \textbf{0.157}&\textbf{0.155}&\textbf{0.160}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-2mm}
\caption{Performance comparisons on the few-shot VDER settings with the CORD dataset.
% And we experiment both the baseline model and an augmented model with hierarchical decoder, annotated as ``Hier''. By adding the DocuNet dataset, we see a signiciant performance boost.
}
\vspace{-4mm}
\label{tab:few-shot}
\end{table*}


==> papers/documentnet/tables/funsd.tex <==
\begin{table}[tp]
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{ccccc}
\hline
         & Precision & Recall & F1-score & Support \\ \hline
Question & 84.84    & 88.41 & 86.59   & 1070    \\
Header   & 57.26    & 56.30 & 56.78   & 119     \\
Answer   & 82.67    & 87.27 & 84.91   & 809     \\ \hline
Average  & 82.41    & 86.04 & \textbf{84.18}   & 1998    \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Detailed metrics on the FUNSD entity extraction task.}
\label{tab:funsd}
\end{table}


==> papers/magvit/sections/0_abstract.tex <==
We introduce the MAsked Generative VIdeo Transformer, \emph{\modelname{}}, to tackle various video synthesis tasks with a single model.
%
%MH: this sentence is redudant as you already mention in the previous sentence. %Lijun: agreed
%We train a single \modelname{} model and apply it to multiple video generation tasks at inference time.
% To achieve this goal, 
With the 3D tokenizer introduced in \cref{chap:3dvq}, we propose an embedding method for masked video token modeling to facilitate multi-task learning.
%
We conduct extensive experiments to demonstrate the quality, efficiency, and flexibility of \modelname{}.
%
Our experiments show that (i) \modelname{} performs favorably against state-of-the-art approaches and establishes the best-published FVD on three video generation benchmarks, including the challenging Kinetics-600. 
%
(ii) \modelname{} outperforms existing methods in inference time by  two orders of magnitude against diffusion models and by 60$\times$ against autoregressive models. 
%
(iii) A single \modelname{} model supports ten diverse generation tasks and generalizes across videos from different visual domains.
%
%We will open source our framework and models.
The source code and trained models are released to the public at \url{https://magvit.cs.cmu.edu}.


==> papers/magvit/tables/cg.tex <==
\begin{table}[tp]
\centering
% \scriptsize
\begin{tabular}{@{}lcccc@{}}
\toprule
Method        & Extra Video  & Class      & FVD$\downarrow$          & IS$\uparrow$                \\ \midrule
% VGAN\cite{vondrick2016generating}  & \checkmark & -                        & 8.31\scriptsize{$\pm$0.09}  \\
% TGAN\cite{saito2017temporal} &            & -                        & 11.85\scriptsize{$\pm$0.07} \\
% MoCoGAN$^\#$\cite{tulyakov2018mocogan} & \checkmark & -                        & 12.42\scriptsize{$\pm$0.07} \\
% ProgressiveVGAN\cite{acharya2018towards}& \checkmark & -                        & 14.56\scriptsize{$\pm$0.05} \\
% TGAN\cite{saito2017temporal} & \checkmark & -                        & 15.83\scriptsize{$\pm$0.18} \\
RaMViD\cite{hoppe2022diffusion}    & &    &   -  &  21.71\mytiny{$\pm$0.21}  \\
% LDVD-GAN\cite{kahembwe2020lower} &            & -                        & 22.91\mytiny{$\pm$0.19} \\
% VideoGPT\cite{yan2021videogpt} &            & -                        & 24.69\mytiny{$\pm$0.30} \\
StyleGAN-V$^{*}$\cite{skorokhodov2022stylegan} & & &-& 23.94\mytiny{$\pm$0.73} \\
% TGANv2\cite{saito2020train} & \checkmark & 1209\mytiny{$\pm$28} & 28.87\mytiny{$\pm$0.67} \\
% MoCoGAN-HD$^*$\cite{tian2021good} & &            & 838                      & 32.36                       \\
% DIGAN\cite{yu2022generating}  & &            & 655\mytiny{$\pm$22}  & 29.71\mytiny{$\pm$0.53} \\
DIGAN\cite{yu2022generating} & &            & 577\mytiny{$\pm$21}  & 32.70\mytiny{$\pm$0.35} \\
DVD-GAN\cite{clark2019adversarial} & & \checkmark & -                        & 32.97\mytiny{$\pm$1.70}  \\
Video Diffusion$^*$\cite{ho2022video} &  &            & -                        & 57.00\mytiny{$\pm$0.62}    \\
TATS\cite{ge2022long}  & &            & 420\mytiny{$\pm$18}  & 57.63\mytiny{$\pm$0.24} \\
CCVS+StyleGAN\cite{le2021ccvs} & &            & 386\mytiny{$\pm$15}  & 24.47\mytiny{$\pm$0.13} \\
Make-A-Video$^*$\cite{singer2022make} & & \checkmark & 367 & 33.00 \\
TATS\cite{ge2022long} & & \checkmark & 332\mytiny{$\pm$18}  & 79.28\mytiny{$\pm$0.38} \\ \midrule
\color{mygray}CogVideo$^*$\cite{hong2022cogvideo} & \color{mygray}\checkmark  & \color{mygray}\checkmark & \color{mygray}626                      & \color{mygray}50.46                       \\
\color{mygray}Make-A-Video$^*$\cite{singer2022make} & \color{mygray}\checkmark & \color{mygray}\checkmark & \color{mygray}81 & \color{mygray}82.55 \\ \midrule
\emph{\modelname}-B-CG (ours) &  & \checkmark & \underline{159\mytiny{$\pm$2}} & \underline{83.55\mytiny{$\pm$0.14}}     \\
\emph{\modelname}-L-CG (ours) & & \checkmark & \textbf{76\mytiny{$\pm$2}}     & \textbf{89.27\mytiny{$\pm$0.15}}     \\ \bottomrule
\end{tabular}
\vspace{-1mm}
\caption{\textbf{Generation performance on the UCF-101 dataset.} 
Methods in \textcolor{mygray}{gray} are pretrained on additional large video data.
% , while the others are only trained on UCF-101 videos.
% Methods with $\checkmark$ in the All column additionally use the UCF-101 test set in training, while the others only use the training set.
Methods with $\checkmark$ in the Class column are class-conditional, while the others are unconditional.
% Methods marked with $^*$ additionally use the test set in training. 
Methods marked with $^*$ use custom resolutions, while the others are at 128$\times$128. 
See Appendix C for more comparisons with earlier works.}
\label{tab:ucf}
\vspace{-4mm}
\end{table}


==> papers/magvit/tables/efficiency.tex <==
% \begin{table}[!ht]
% \caption{Inference efficiency. \lijun{Needs verification}}
% \label{tab:efficiency}
% \centering
% \begin{tabular}{@{}lccc@{}}
% \toprule
% Method               & \makecell{Sequence\\length}    & \#Steps$\downarrow$ & Complexity $\downarrow$ \\ \midrule
% % CogVideo\cite{hong2022cogvideo} & 4096  & 4096 &   \\
% % CCVS\cite{le2021ccvs} & 4096  & 4096 &   \\
% % VideoGPT\cite{yan2021videogpt} & 8192 &    8192    &               \\
% % Transframer\cite{nash2022transframer} & 4096 &  4096  &                \\
% % N\"UWA\cite{wu2021n}  & 7056  & 7056  &        \\
% % RaMViD\cite{hoppe2022diffusion} & - &  1000   &   \\
% Video Diffusion\cite{ho2022video} & - & 256-512  & $\gO(THWK)$   \\ 
% TATS\cite{ge2022long} & 1024 & 1024 & $\gO(T^3H^3W^3)$ \\
% MaskViT\cite{gupta2022maskvit} & 4096 & 16-64  &    $\gO(T^2H^2W^2K)$           \\\midrule
% \modelname{}  (ours) &  1024 & 12  & $\gO(T^2H^2W^2K)$       \\ \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[tp]
\scriptsize
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
Method               & \makecell{Seq.\\length$\downarrow$}    & \# Steps$\downarrow$ & \makecell{Estimated\\Relative\\Runtime$\downarrow$} \\ \midrule
Video Diffusion\cite{ho2022video} & - & 256-512  & $\gg$250 \\ 
TATS\cite{ge2022long} & 1024 & 1024 & 60  \\
MaskViT\cite{gupta2022maskvit} & 4096 & 16-64  &   4-12   \\\midrule
\emph{\modelname}  (ours) &  \textbf{1024} & \textbf{12}  &   \textbf{1}   \\\bottomrule
\end{tabular}
\caption{\textbf{Comparison of key properties for inference efficiency.}}
\label{tab:efficiency}
\end{table}


==> papers/magvit/tables/fp.tex <==
\begin{table}[tp]
\centering
\scriptsize
\begin{tabular}{@{}lcc@{}}
\toprule
Method                   & K600 FVD$\downarrow$   & BAIR FVD$\downarrow$ \\ \midrule
% LVT\cite{rakhimov2021latent} & 224.7                      & 126\scriptsize{$\pm$3} \\
% Video Transformer\cite{weissenborn2019scaling} & 170.0\scriptsize{$\pm$5.0} & 94\scriptsize{$\pm$2}  \\
CogVideo\cite{hong2022cogvideo}  & 109.2                      & -                      \\
% DVD-GAN-FP\cite{clark2019adversarial} & 69.1\scriptsize{$\pm$1.2}  & 110                    \\
CCVS\cite{le2021ccvs}    & 55.0\mytiny{$\pm$1.0}  & 99\mytiny{$\pm$2}  \\
Phenaki\cite{villegas2022phenaki} & 36.4\mytiny{$\pm$0.2} & 97 \\
% VideoGPT\cite{yan2021videogpt}  & -                          & 103                    \\
TrIVD-GAN-FP\cite{luc2020transformation} & 25.7\mytiny{$\pm$0.7}  & 103                    \\
Transframer\cite{nash2022transframer}  & 25.4                       & 100                    \\
MaskViT\cite{gupta2022maskvit} & -                          & 94                     \\
FitVid\cite{babaeizadeh2021fitvid} & -                          & 94                     \\
MCVD\cite{voleti2022masked} & - & 90 \\
N\"UWA\cite{wu2021n}    & -                          & 87                     \\
RaMViD\cite{hoppe2022diffusion}        &  16.5     &   84 \\
Video Diffusion\cite{ho2022video}  & \underline{16.2\mytiny{$\pm$0.3}}  & -                     \\ \midrule
\emph{\modelname}-B-FP (ours)          & 24.5\mytiny{$\pm$0.9}     & \underline{76{\mytiny$\pm$0.1}} (48{\mytiny$\pm$0.1})   \\
\emph{\modelname}-L-FP (ours)         & \textbf{9.9\mytiny{$\pm$0.3}}     & \textbf{62{\mytiny$\pm$0.1}}  (31{\mytiny$\pm$0.2})   \\ \bottomrule
\end{tabular}
\vspace{-1mm}
\caption{\textbf{Frame prediction performance on the BAIR and Kinetics-600 datasets.} 
%Values marked with $^*$ use the new evaluation protocol on BAIR with uniformly sampled test clips. 
- marks that the value is unavailable in their paper or incomparable to others.
The FVD in parentheses uses a debiased evaluation protocol on BAIR detailed in Appendix B.3.
% \lu{add details in comparison in the appendix.}
% that uniformly samples test clips.
%The best values for each metric are in bold, while the second best are in italic.
See Appendix C for more comparisons with earlier works.
}
\label{tab:bairk600}
% \vspace{-2mm}
\end{table}



==> papers/magvit/tables/mt_bair.tex <==
\begin{table*}[tp]
\centering
\scriptsize
\begin{tabular}{@{}lc|ccccccccc|cccc@{}}
\toprule
Method &Task &\textbf{BAIR-MT8}$\downarrow$ & FP & FI & OPC & OPV & OPH & OPD & IPC & IPD & \textbf{SSV2-MT10}$\downarrow$ & CG & CFP \\ \midrule
\modelname-B-UNC &Single& 150.6 & {\color{mygray}74.0} & {\color{mygray}71.4} & {\color{mygray}119.0} & {\color{mygray}46.7} & {\color{mygray}55.9} & {\color{mygray}389.3} & {\color{mygray}145.0} & {\color{mygray}303.2} & 258.8 & {\color{mygray}107.7} & {\color{mygray}279.0}  \\
\modelname-B-FP  & Single &201.1 & 47.7 & {\color{mygray}56.2}& {\color{mygray}247.1} & {\color{mygray}118.5} & {\color{mygray}142.7}  & {\color{mygray}366.3} & {\color{mygray}357.3} & {\color{mygray}272.7} & 402.9 & {\color{mygray}1780.0} & 59.3 \\ \hdashline
\modelname-B-\emph{MT} & Multi& 32.8 & 47.2 & 36.0 & 28.1 & 29.0 & 27.8 & 32.1 & 31.1 & 31.0 & 43.4 & 94.7 & 59.3     \\
\modelname-L-\emph{MT} & Multi& \textbf{22.8} & 31.4 & 26.4 & 21.3 & 21.2 & 19.5 & 20.9 & 21.3 & 20.3 & \textbf{27.3} & 79.1 & 28.5  \\\bottomrule
\end{tabular}
\vspace{-1mm}
\caption{\textbf{Multi-task generation performance on BAIR and SSV2 evaluated by FVD.} \textcolor{mygray}{Gray} values denote unseen tasks during training. We list per-task FVD for all eight tasks on BAIR and the two extra tasks on SSV2 here, and leave the details for SSV2 in Appendix C.}
\label{tab:mt_bair}
% \vspace{-2mm}
\end{table*}

% \begin{table*}[!ht]
% \centering
% \caption{Comparison between different condition methods.}
% \label{tab:multitask}
% \begin{tabular}{@{}cccccccccccc@{}}
% \toprule
% Method & MT & \textbf{Avg}$\downarrow$ & FP & FI & OPV & OPH & OPC & OPD & IPC & IPD \\ \midrule
% Unconditional &  & 150.6 & {\color{mygray}74.0} & {\color{mygray}71.4} & {\color{mygray}46.7} & {\color{mygray}55.9} & {\color{mygray}119.0} & {\color{mygray}389.3} & {\color{mygray}145.0} & {\color{mygray}303.2}  \\
% Prefix & \checkmark &  1827 & {\color{mygray}1096} & {\color{mygray}2466} & {\color{mygray}1435} & {\color{mygray}1957} & {\color{mygray}1259} & {\color{mygray}1966} &  {\color{mygray}2116}  & {\color{mygray}2318}     \\
% Prefix+replace & \checkmark & 76.3 & 48.5 & 43.9 & 37.0 & 42.1 & 39.4 & 275.8 & 47.3 & 76.8  \\ \midrule
% Prefix+repredict &  & -  & 47.6  & {\color{mygray}-} & {\color{mygray}-} & {\color{mygray}-} & {\color{mygray}-} & {\color{mygray}-} & {\color{mygray}-} & {\color{mygray}-}  \\
% COMMIT &  & 201.1 & 47.7 & 56.2 & {\color{mygray}118.5} & {\color{mygray}142.7} & {\color{mygray}247.1} & {\color{mygray}366.3} & {\color{mygray}357.3} & {\color{mygray}272.7}  \\
% COMMIT & \checkmark & 32.8 & 47.2 & 36.0 & 29.0 & 27.8 & 28.1 & 32.1 & 31.1 & 31.0     \\
% \end{tabular}
% \end{table*}


==> papers/magvit/tables/task_mask.tex <==
\begin{table}[!h]
\centering
\scriptsize
\begin{tabular}{@{}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{}}
\toprule
& CG & FP & CFP & FI & OPC & OPV & OPH & OPD  & IPC  & IPD \\ \midrule
Masked pixel & 100\% & 94\% & 94\% & 87\% & 75\% & 50\% & 50\% & 50\% & 25\% & 25\% \\
Masked token & 100\% & 75\% & 75\% & 50\% & 75\% & 50\% & 50\% & 50\% & 25\% & 25\% \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\caption{Proportions of masked pixels and tokens for each task.}
\label{tab:task_mask}
\vspace{-4mm}
\end{table}

==> papers/magvit/tables/tasks.tex <==
\begin{table}[tp]
\centering
\scriptsize
\begin{tabular}{@{}lcc@{}}
\toprule
Task & \makecell{Condition Pixels} & \makecell{Fully Masked\\Input Tokens} \\ \midrule
\makecell[cl]{\textbf{CG}:\\Class-conditional\\Generation}   & \makecell{\includegraphics[width=.2\linewidth]{fg_vid}} & \makecell{\includegraphics[width=.2\linewidth]{fg_tok}}  \\
\makecell[cl]{\textbf{FP}:\\Frame\\Prediction}   & \makecell{\includegraphics[width=.2\linewidth]{fp_vid}} & \makecell{\includegraphics[width=.2\linewidth]{fp_tok}}  \\
\makecell[cl]{\textbf{CFP}:\\Class-conditional\\Frame Prediction}   & \makecell{\includegraphics[width=.2\linewidth]{fp_vid}} & \makecell{\includegraphics[width=.2\linewidth]{cfp_tok}}  \\
\makecell[cl]{\textbf{FI}:\\Frame\\Interpolation}   & \makecell{\includegraphics[width=.2\linewidth]{fi_vid}} & \makecell{\includegraphics[width=.2\linewidth]{fi_tok}}  \\
\makecell[cl]{\textbf{OPV}:\\Vertical\\Out Painting}   & \makecell{\includegraphics[width=.2\linewidth]{opv_vid}} & \makecell{\includegraphics[width=.2\linewidth]{opv_tok}}  \\
\makecell[cl]{\textbf{OPH}:\\Horizontal\\Outpainting}   & \makecell{\includegraphics[width=.2\linewidth]{oph_vid}} & \makecell{\includegraphics[width=.2\linewidth]{oph_tok}}  \\
\makecell[cl]{\textbf{OPC}:\\Central\\Out Painting}   & \makecell{\includegraphics[width=.2\linewidth]{opc_vid}} & \makecell{\includegraphics[width=.2\linewidth]{opc_tok}}  \\
\makecell[cl]{\textbf{OPD}:\\Dynamic\\Outpainting}   & \makecell{\includegraphics[width=.2\linewidth]{opd_vid}} & \makecell{\includegraphics[width=.2\linewidth]{opd_tok}}  \\
\makecell[cl]{\textbf{IPC}:\\Central\\Inpainting}   & \makecell{\includegraphics[width=.2\linewidth]{ipc_vid}} & \makecell{\includegraphics[width=.2\linewidth]{ipc_tok}}  \\
\makecell[cl]{\textbf{IPD}:\\Dynamic\\Inpainting}   & \makecell{\includegraphics[width=.2\linewidth]{ipd_vid}} & \makecell{\includegraphics[width=.2\linewidth]{ipd_tok}}  \\ \bottomrule
\end{tabular}
\caption{Task list with condition definition in pixel and token spaces. Condition pixels are in green, while paddings are in white. Condition tokens are in yellow and \mask tokens are in gray. An orange token indicates provided class index as prefix condition, while a white token indicates a \texttt{[NOCLASS]} token. \lu{The third column looks naive without much information. Consider making it two column table and add code for padding.}}
\label{tab:task}
\end{table}

==> papers/magvit/tables/token2.tex <==
\begin{table}[!h]
\centering
\scriptsize
\begin{tabular}{l@{\hspace{6pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{7pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{7pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c}
\toprule
\multirow{2}{*}{VQ Tokenizer} & \multicolumn{3}{l}{From Scratch} & \multicolumn{6}{c}{ImageNet Initialization} \\
& P$\uparrow$ & S$\uparrow$ & L$\downarrow$ & P$\uparrow$ & S$\uparrow$  & L$\downarrow$ & P$\uparrow$ & S$\uparrow$ & L$\downarrow$ \\ \midrule
MaskGIT 2D  &
 21.4 & 0.667 & 0.139 & 21.5 & 0.685 & 0.114 & \multicolumn{3}{c}{-} \\
% TATS 3D & 
% 23.2 & 0.784 &  & \multicolumn{3}{c}{-}& \multicolumn{3}{c}{-} \\ 
\midrule
& & & & \multicolumn{3}{c}{Average} & \multicolumn{3}{c}{Central} \\
% \emph{\modelname{}} 3D-VQ-B & 
% 20.7 & 0.640 & 0.143 & 21.1 & 0.662 & 0.123 & 21.3 & 0.673 & 0.113 \\ 
\emph{\modelname{}} 3D-L &
21.8 & 0.690 & 0.113 & 21.9 & 0.697 & 0.103 & \textbf{22.0} & \textbf{0.701} & \textbf{0.099} \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\caption{\textbf{Image quality metrics of different tokenizers} on UCF-101 training set reconstruction.
P: PSNR, S: SSIM, L: LPIPS.
}
\label{tab:token_imquality}
\vspace{-4mm}
\end{table}


==> papers/magvitv2/sections/related.tex <==
%\vspace{-4mm}
% \paragraph{Visual tokenization.}
%Mapping visual inputs to compact discrete representations is a longstanding goal in machine learning.
Beyond the VQ-VAE models discussed above, additional models have been proposed. ViT-VQGAN \cite{yu2021vector} introduces transformer blocks as a substitute for CNNs for image tokenization. C-ViViT \cite{villegas2022phenaki} further extends this idea for video tokenization. %Tokenizing video is more complex since it requires modeling the visual dynamics within the compressed spatial-temporal latent space. 
Early studies on video tokenization treat frames as independent images with no temporal compression~\cite{wu2021n,gupta2022maskvit}. Later research \cite{yan2021videogpt,ge2022long,yu2022magvit} integrates 3D CNNs to tokenize spatial-temporal volumes. Despite these advances in vector quantization (VQ), the codebook learned by previous VQ models is relatively small (\eg, $8$k) due to the difficulty in improving the generation quality with larger vocabularies. In contrast, our tokenizer can induce a large vocabulary (\eg, $262$k) that can be effectively modeled by an LM, leading to enhanced image and video generation quality. 


% In the deep learning era, VQVAE \cite{van2017neural} shows the first learned discrete representations that outperform continuous ones for image generation, by proposing an extension of the VAE \cite{kingma2013auto} that uses a learned codebook for latent embedding quantization. VQGAN \cite{esser2021taming} extends the VQVAE with adversarial and perceptual losses to mitigate the blurriness induced by the reconstruction loss. While the original VQVAE used a PixelCNN \cite{van2016conditional} to model the prior of discrete latents, \cite{esser2021taming} use a language model for this task, achieving high resolution image generation.  




% While it is possible to tokenize each frame in a video separately as an image \cite{wu2021n},  TATS \cite{ge2022long} and MAGVIT \cite{yu2022magvit} incorporate 3D convolutional filters in the encoder and decoder of the VQGAN to tokenize videos as a whole. ViT-VQGAN \cite{yu2021vector} for images, and  C-ViViT \cite{villegas2022phenaki} for videos, show it is also possible to use a transformer backbone instead of a CNN for the VQGAN. 

% An intuitive solution is to simply decompose the codebook into several chunks along the channel dimension~\cite{rakhimov2021latent}, but this results in even longer sequences.

%\vspace{-4mm}
\paragraph{Text-to-\{image, video\}.}
Text-to-image and text-to-video generation has garnered significant rapid advancements using both language models~\cite{yu2023scaling,chang2023muse} and diffusion models~\cite{ho2022imagen,blattmann2023align,singer2022make,ge2023preserve,ramesh2022hierarchical}. Although diffusion models, such as Midjourney, are considered the top performers in these tasks, it is unclear whether their advantage stems from the model, data, or some other unidentified factors. Indeed, it is challenging to scientifically compare these text-to-image models as they are trained on varied datasets, with some even being proprietary data, under inconsistent training conditions. To facilitate a fairer comparison, this paper prioritizes using the ImageNet and Kinetics benchmarks.
% We are training text-to-video models which may be ready by the next revision.

%\vspace{-4mm}
\paragraph{Diffusion models.}
Exhibiting high quality sampling, pixel-space diffusion models \cite{sohl2015deep,song2019generative,ho2020denoising} raised to the top of the generative modeling space for both image \cite{ho2020denoising,dhariwal2021diffusion,saharia2022photorealistic} and video \cite{ho2022video,ho2022imagen,singer2022make} synthesis. The pixel-space denoising diffusion models (DDMs) are later refined by the latent-space DDM \cite{rombach2022high}, which conducts diffusion over the \emph{continuous} latent embeddings derived from a pre-trained variational autoencoder (VAE).
Binary latents for image modeling were used in \cite{wang2023binary}, where the diffusion process is parameterized with Bernoulli distributions.
%The stable diffusion model is a prominent example of latent DDM.
% Latent diffusion models for images \cite{rombach2022high} utilize the same modeling principle, but instead of pixel values model the distribution of.
%Conversely, while the U-Net~\cite{ronneberger2015u} has been the common neural architecture for both pixel- and latent-space diffusion models, 
Recent studies have identified advantages in substituting the U-Net~\cite{ronneberger2015u} denoising backbone with a Transformer \cite{peebles2022scalable,jabri2023scalable} or a hybrid of both \cite{hoogeboom2023simple}, making the distinctions between diffusion and language models in visual generation more blurred, with a key distinction being their latent format — continuous for diffusion and discrete for language models.
%Specifically, both DDM and MLM emulate a gradual corruption process on the latents and generate samples through iterative denoising restoration.
%In this paper we demonstrate that discrete latent space modeling outperforms all the compared continuous diffusion approaches, both in sampling quality and efficiency, when utilizing an appropriate visual tokenizer.




==> papers/magvitv2/tables/generation_ar.tex <==
\begin{table}[tp]
\centering
% \vspace{-6mm}
\caption{\cl{\textbf{Video generation results}: class-conditional generation on UCF-101 with AR-LM models. We use the same transformer configuration as MLM experiments but without vocabulary factorization and weight tying. As a result, the AR-LM with \modelname{} uses more parameters in the embedding table and the softmax layer.}
% \emph{Method types}: AutoRegressive Language Model (ARLM), Masked Language Model (MLM), Generative Adversarial Network (GAN), continuous Diffusion (Diff.). 
% \emph{Latent types}: \quantizerfullname{} (\quantizername{}), Vector Quantization (VQ), Variational AutoEncoder (VAE), Discrete Cosine Transformation (DCT). 
% We report the bits per pixel (bpp) of the representation used in each latent-space model.
}
\label{tab:gen_ar}
% \vspace{-2mm}
% \resizebox{\linewidth}{!}{%
\centering
\cl{\begin{tabular}{@{}llcc@{}}
\toprule
Tokenizer   & FVD$\downarrow$  & \#Params  & \#Steps  \\ \midrule
MAGVIT~\cite{yu2022magvit} & 265  & 306M & 1024 \\
% &      MLM  & 76 & 306M   & 12  \\ \hdashline
\emph{\modelname{} (ours)} & \textbf{109}  & 840M & 1280\\
%  & MLM &  \textbf{58}  & 307M & 12  \\
\bottomrule
\end{tabular}
}
% \vspace{-2mm}
% }
\end{table}



==> papers/magvitv2/tables/generation_bk2.tex <==
\begin{table}[p]
\centering
\caption{\textbf{Video and image generation results}. 
\emph{Method types}: AutoRegressive Language Model (ARLM), Masked Language Model (MLM), Generative Adversarial Network (GAN), continuous Diffusion (Diff.). 
\emph{Latent types}: \quantizerfullname{} (\quantizername{}), Vector Quantization (VQ), Variational AutoEncoder (VAE), Discrete Cosine Transformation (DCT). guidance indicates the classifier-free diffusion guidance.
We report the bits per pixel (bpp) of the representation used in each latent-space model.
$^*$ indicates usage of extra training data.
}
\label{tab:generation}
\vspace{-2mm}
\begin{subtable}{\linewidth}
\caption{Frame prediction on Kinetics-600 and class-conditional generation on UCF-101.}
\label{tab:gen_k600_full}
\vspace{-2mm}
\resizebox{\linewidth}{!}{%
\centering
\begin{tabular}{@{}l@{\hspace{5pt}}l@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{3pt}}c@{\hspace{5pt}}c@{}}
\toprule
Type & Method   & K600 FVD$\downarrow$  & UCF FVD$\downarrow$  & \#Params  & \#Steps &  \\ \midrule
\multicolumn{5}{l}{\textit{Pixel-Space Generative Models}} \\
ARLM & Video Transformer~\cite{weissenborn2019scaling} & 170.0\mytiny{$\pm$5.0} & & 373M & 197k  \\
GAN & DVD-GAN-FP~\cite{clark2019adversarial}  & 69.1\mytiny{$\pm$1.2} & & & 1                    \\
GAN & TrIVD-GAN-FP~\cite{luc2020transformation}  & 25.7\mytiny{$\pm$0.7} &  & & 1                \\
Diffusion & RaMViD~\cite{hoppe2022diffusion}   &  17.5\mytiny{$\pm$1.1} & & 308M & 1000  \\
Diffusion & Video Diffusion~\cite{ho2022video}  & 16.2\mytiny{$\pm$0.3} & & 1.1B &   256        \\
Diffusion & RIN~\cite{jabri2023scalable} & 10.8 & & 411M & 1000 \\
\midrule
\multicolumn{6}{l}{\textit{Latent-Space Generative Models}} & Latent bpp\\
ARLM + VQ & LVT~\cite{rakhimov2021latent} & 224.7 &  & 50M  & 16k & 2.000 \\
ARLM + VQ & CogVideo$^*$~\cite{hong2022cogvideo}  & 109.2 & 626 & 9.4B   & 64k & 0.223$^*$        \\
ARLM + VQ & CCVS~\cite{le2021ccvs}   & 55.0\mytiny{$\pm$1.0} & 386\mytiny{$\pm$18} & 361M   & 1024& 0.219 \\
ARLM + VQ & TATS~\cite{ge2022long}  &  & 332\mytiny{$\pm$18} & 321M & 1024 &  0.055 \\
MLM + VQ & Phenaki~\cite{villegas2022phenaki} & 36.4\mytiny{$\pm$0.2} & & 227M   & 48 & 0.406\\
ARLM + DCT & Transframer~\cite{nash2022transframer}  & 25.4  &  & 662M &  $<$4k    & $\approx$6   \\
% T MAGVIT-B-FP        & 24.5\mytiny{$\pm$0.9}     & 43.3\mytiny{$\pm$1.8} & 88M & 0.039 & 12 \\
MLM + VQ & MAGVIT~\cite{yu2022magvit}        & 9.9\mytiny{$\pm$0.3} & 76\mytiny{$\pm$2} & 306M   & 12 & 0.039 \\ 
\hdashline
\multirow{2}{*}{MLM + \quantizername{}} & \multirow{2}{*}{\emph{\modelname{} (ours)}} & 5.2\mytiny{$\pm$0.2} &  & \multirow{2}{*}{307M} & 12 & \multirow{2}{*}{0.070} \\
 & & \textbf{4.3\mytiny{$\pm$0.1}}  & \textbf{58\mytiny{$\pm$3}} & & 24 &  \\
\bottomrule
\end{tabular}
}
\end{subtable}

\begin{subtable}{\linewidth}
\vspace{2mm}
\caption{Class-conditional image generation on ImageNet 512$\times$512.
% \lu{we can remove GAN.} \lijun{recent diffusion papers all kept those, esp. StyleGAN-XL which is very strong}
}
\label{tab:gen_in512_full}
\vspace{-2mm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l@{\hspace{5pt}}l@{\hspace{4pt}}c@{\hspace{2pt}}c@{\hspace{3pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{5pt}}c@{}}
\toprule
\multirow{2}{*}{Type}  & \multirow{2}{*}{Method}  & \multicolumn{2}{c}{w/o guidance} & \multicolumn{2}{c}{w/ guidance}  & \multirow{2}{*}{\#Params}  & \multirow{2}{*}{\#Steps} &  \\
& & FID$\downarrow$ & IS$\uparrow$ & FID$\downarrow$ & IS$\uparrow$ \\ \midrule
% \multicolumn{6}{l}{\textbf{512 $\times$ 512 resolution}} \\
\multicolumn{6}{l}{\textit{Pixel-Space Generative Models}} \\
% ADM & & 23.24 & 58.06 & 7.72 & 172.71 \\
Diffusion & ADM+Upsample~\cite{dhariwal2021diffusion}  & 9.96  & 121.8 & 3.85 & 221.7 & 731M & 2000 \\
GAN & BigGAN-deep~\cite{brock2018large} & 8.43 & 177.9 & & & 160M  & 1 \\
Diffusion & RIN~\cite{jabri2023scalable} & 3.95 & 216.0 & & & 320M  & 1000 \\
Diffusion & simple diffusion~\cite{hoogeboom2023simple} & 3.54 & 205.3 & 3.02 & 248.7 & 2B & 512 &\\
Diffusion & VDM++~\cite{kingma2023vdm}  & 2.99 & 232.2 & 2.65 & 278.1  & 2B & 512 \\
GAN & StyleGAN-XL~\cite{sauer2022stylegan} & & & 2.41 & 267.8 & 168M & 1 \\
\midrule
\multicolumn{8}{l}{\textit{Latent-Space Generative Models}} & Latent bpp \\
Diff. + VAE & DiT-XL/2~\cite{peebles2022scalable} & 12.03 & 105.3 & 3.04 & 240.8 & 675M  & 250 & 2.000$^*$ \\
 
MLM + VQ & MaskGIT~\cite{chang2022maskgit} & 7.32 & 156.0 & & & 227M & 12  & 0.039 \\
MLM + VQ & Token-Critic~\cite{lezama2022improved} & 6.80 & 182.1 &  &  & 368M & 36 & 0.039 \\
MLM + VQ & DPC+Upsample~\cite{lezama2022discrete}  & 3.62 & 249.4 & & & 619M & 72 & 0.039   \\
% MLM + VQ & DPC-light(5)+U~\cite{lezama2022discrete}  & 3.62 & 249.40 & & & 619M & 72 & 0.039   \\
\hdashline
\multirow{2}{*}{MLM + \quantizername{}} & \multirow{2}{*}{\emph{\modelname{} (ours)}} & 4.61 & 192.4 & & & \multirow{2}{*}{307M} & 12 & \multirow{2}{*}{\textbf{0.018}} \\
& & 3.07 & 213.1 & \textbf{1.91} & \textbf{324.3} &  & 64 & \\
% & \emph{\modelname{} (ours)} (40 bits) &  & & &  & 312M & & 0.039 \\
\bottomrule
\end{tabular}}
\end{subtable}

\end{table}


==> papers/spae/tables/miniimagenet_2way_full.tex <==
\begin{table}[tp]
% \vspace{-4mm}
\centering
\caption{\textbf{Few-shot classification accuracy} on the mini-ImageNet 2-way benchmarks.}
\label{tab:imagenet_2way_full}
% \small
\begin{tabular}{@{}lllcccccccc@{}}
\toprule
\multicolumn{3}{r}{Task Induction} &    & \checkmark & \checkmark& \checkmark& \checkmark& \checkmark& \checkmark & \multirow{3}{*}{Avg} \\
Method &\# Layers & \multicolumn{1}{r}{Inner Shots}   & 1    & 1    & 3    & 5    & 1    & 1    & 1    &                      \\
& :\ \# Tokens & \multicolumn{1}{r}{Repeats}         & 0    & 0    & 0    & 0    & 1    & 3    & 5    &                      \\
\midrule
% Frozen~\cite{tsimpoukelli2021multimodal} &- &   & 1.7  & 33.7 & 66   & 66   & 63   & 65   & 63.7 & 51.3                 \\
LQAE~\cite{liu2023language} & 1: 256 & GPT 3.5 & 1.5  & 35.2 & 68.2 & 69.8 & 68.5 & 68.7 & 65.9 & 53.97                \\ \midrule
% $\emph{\modelname{}}_\text{GPT}$ (ours) &2: 5& GPT 3.5 & \textit{5.3} &  \textit{77.2}    &   \textit{84.4}   &    \textit{86.0}  & \textit{79.4} & \textit{77.2}  & \textit{77.1}    &    \textit{69.51}                  \\ \midrule
\emph{\modelname{}}$_\text{PaLM}$ & 1: 1 & PaLM 2  & \textbf{34.8} & 77.2 & 81.2 & 80.3 & 74.0 & 73.2 & 71.5 & 70.31                \\
\emph{\modelname{}}$_\text{PaLM}$ & 2: 5 & PaLM 2  & 32.2 & 84.0 & 88.5 & 88.4 & \textbf{85.1} & 83.6 & 82.4 & 77.74                \\
\emph{\modelname{}}$_\text{PaLM}$ & 3: 21 & PaLM 2  & 27.9 & \textbf{84.8} & \textbf{92.5} & \textbf{92.6} & 84.8 & \textbf{85.2} & \textbf{85.4} & \textbf{79.03}                \\ 
\emph{\modelname{}}$_\text{PaLM}$ & 4: 85 & PaLM 2  & 22.8 & 81.1 & 91.4 & 90.4 & 82.6 & 84.3 & 84.7 & 76.76               \\
\emph{\modelname{}}$_\text{PaLM}$ & 5: 341 & PaLM 2  & 21.2 & 77.4 & 88.0 & 79.1 & 84.8 & 74.0 & 76.1 & 71.51               \\
\emph{\modelname{}}$_\text{PaLM}$ & 6: 597 & PaLM 2  & 21.8 & 73.8 & 70.8 & 62.4 & 64.8 & 62.1 & 58.6 & 59.19               \\ \midrule
\emph{\modelname{}}$_\text{PaLM}^\text{disjoint}$ & 2: 5 & PaLM 2 & 24.8 & 79.8 & 84.5 & 83.7 & 80.8 & 78.5 & 78.4 & 72.93 \\
\emph{\modelname{}}$_\text{PaLM}^\text{disjoint}$ & 3: 21 & PaLM 2  & 21.4 & 81.4 & 89.2 & 87.9 & 82.6 & 81.7 & 80.6 & 74.98                \\ 
% $\emph{\modelname{}}_\text{PaLM}$ (Ours) & PaLM v2 & \textbf{34.8} & \textbf{84.8} & \textbf{92.5} & \textbf{92.6} & \textbf{85.1} & \textbf{85.2} & \textbf{85.4} & \textbf{80.06}  \\   
% & \makecell(r){$d=$} & $1$ & $3$ & $3$ & $3$ & $2$ & $3$ & $3$ \\ 
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}


==> papers/spae/tables/miniimagenet_5way.tex <==
\begin{table}[tp]
% \vspace{-6mm}
\centering
\caption{\textbf{Few-shot classification accuracy} on the mini-ImageNet 5-way benchmarks.}
\label{tab:imagenet_5way}
\small
\begin{tabular}{@{}lllcccccccc@{}}
\toprule
\multicolumn{3}{r}{Task Induction} & & \checkmark & \checkmark& \checkmark& \checkmark& \checkmark& \checkmark & \multirow{3}{*}{Avg} \\
Method  &\# Layers & \multicolumn{1}{r}{Inner Shots}    & 1            & 1             & 3             & 5             & 1             & 1             & 1             &                      \\
& : \# Tokens & \multicolumn{1}{r}{Repeats}        & 0            & 0             & 0             & 0             & 1             & 3             & 5             &                      \\ 
\midrule
Frozen~\cite{tsimpoukelli2021multimodal} &- &     & 0.9          & 14.5          & 34.7          & 33.8          & 33.8          & 33.3          & 32.8          & 26.26                \\ \midrule
LQAE~\cite{liu2023language} & 1: 256 & GPT 3.5 & 1            & 15.7          & 35.9          & 36.5          & 31.9          & 36.4          & 45.9          & 29.04                \\
$\emph{\modelname{}}_\text{GPT}$ (ours) &2: 5& GPT 3.5 & \textit{4.3} &  \textit{63.0}    &   \textit{63.4}   &    \textit{60.6}  & \textit{61.9} & \textit{62.1}  & \textit{62.1}    &    \textit{53.91}                  \\ \midrule
$\emph{\modelname{}}_\text{PaLM}$ (ours) & 2: 5  & PaLM 2     & \textbf{23.6} & 64.2 & 68.0 & 69.9 & 63.4 & 62.0 & 60.2 & 58.76       \\ 
$\emph{\modelname{}}_\text{PaLM}$ (ours) & 3: 21 & PaLM 2     & 20.2 & \textbf{65.1} & \textbf{73.7} & \textbf{74.3} & \textbf{66.4} & \textbf{67.0} & \textbf{66.3} & \textbf{61.86}       \\ 
% & \makecell[r]{$d=$} & $1$ & $3$ & $3$ & $3$ & $3$ & $3$ & $4$ \\ 
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}

==> papers/spae/tables/miniimagenet_5way_full.tex <==
\begin{table}[tp]
% \vspace{-6mm}
\centering
\caption{\textbf{Few-shot classification accuracy} on the mini-ImageNet 5-way benchmarks. - means value unavailable due to an infeasible sequence length.}
\label{tab:imagenet_5way_full}
% \small
\begin{tabular}{@{}lllcccccccc@{}}
\toprule
\multicolumn{3}{r}{Task Induction} & & \checkmark & \checkmark& \checkmark& \checkmark& \checkmark& \checkmark & \multirow{3}{*}{Avg} \\
Method  &\# Layers & \multicolumn{1}{r}{Inner Shots}    & 1            & 1             & 3             & 5             & 1             & 1             & 1             &                      \\
& : \# Tokens & \multicolumn{1}{r}{Repeats}        & 0            & 0             & 0             & 0             & 1             & 3             & 5             &                      \\ 
\midrule
% Frozen~\cite{tsimpoukelli2021multimodal} &- &     & 0.9          & 14.5          & 34.7          & 33.8          & 33.8          & 33.3          & 32.8          & 26.26                \\
% LQAE~\cite{liu2023language} & 1: 256 & GPT 3.5 & 1            & 15.7          & 35.9          & 36.5          & 31.9          & 36.4          & 45.9          & 29.04                \\ \midrule
% \emph{\modelname (Ours)} & GPT-3.5 &              &               &               &               &               &               &               &                      \\
\emph{\modelname{}}$_\text{PaLM}$ & 1: 1  & PaLM 2     & \textbf{26.8} & 52.0 & 50.9 & 49.9 & 51.9 & 48.4 & 47.9 & 46.83       \\ 
\emph{\modelname{}}$_\text{PaLM}$  & 2: 5  & PaLM 2     & 23.6 & 64.2 & 68.0 & 69.9 & 63.4 & 62.0 & 60.2 & 58.76       \\ 
\emph{\modelname{}}$_\text{PaLM}$  & 3: 21 & PaLM 2     & 20.2 & \textbf{65.1} & \textbf{73.7} & \textbf{74.3} & \textbf{66.4} & \textbf{67.0} & 66.3 & \textbf{61.86}       \\ 
\emph{\modelname{}}$_\text{PaLM}$  & 4: 85  & PaLM 2     & 16.1 & 58.5 & 67.2 & 69.1 & 64.0 & 66.4 & \textbf{67.4} & 58.39       \\ 
\emph{\modelname{}}$_\text{PaLM}$  & 5: 341  & PaLM 2     & 12.1 & 46.3 & 55.9 & 67.2 & 43.3 & 46.3 & - & -      \\ 
\emph{\modelname{}}$_\text{PaLM}$  & 6: 597  & PaLM 2     & 12.1 & 35.7 & - & - & - & - & - & -      \\ 
%\midrule
%\emph{\modelname{}}$_\text{PaLM}^\text{clean}$  & 2: 5 & PaLM 2   & 13.6 & 56.4 & 59.2 & 60.0 & 54.2 & 50.2 & 48.1 & 48.82 \\
%\emph{\modelname{}}$_\text{PaLM}^\text{clean}$  & 3: 21 & PaLM 2   & 10.4 & 57.3 & 62.1 & 62.8 & 56.9 & 55.2 & 51.6 & 50.90 \\
% & \makecell[r]{$d=$} & $1$ & $3$ & $3$ & $3$ & $3$ & $3$ & $4$ \\ 
\bottomrule
\end{tabular}
% \vspace{-4mm}
\end{table}

==> papers/spae/tables/vq_ablation.tex <==
\begin{table}[tp]
% \vspace{-3mm}
\caption{\textbf{Ablation studies} on codebook, semantic guidance, quantization method, and token structure.}
\label{tab:vq_ablation}
\centering
\small
\begin{tabular}{@{}lccccccccc@{}}
\toprule
\multirow{2}{*}{Method} & \# Layers & \multirow{2}{*}{FID$\downarrow$}  & \multirow{2}{*}{IS$\uparrow$}     & \multirow{2}{*}{LPIPS$\downarrow$} & \multirow{2}{*}{CLIP$\uparrow$}   & Relative \\ 
& : \# Tokens & & & & & CLIP$\uparrow$ \\ \midrule
Baseline VQ  & 1: 256 & 5.48 & 119.69 & 0.13  & n/a & n/a       \\
\ \ \ \ + frozen codebook & 1: 256 & 7.44 & 101.39 & 0.17  & 0.1464 & 0.5260   \\
\ \ \ \ \ \ \ \ + semantic guidance & 1: 256 & 5.17 & 124.41 & 0.13  & 0.1518 & 0.5510   \\ \midrule
\multirow{2}{*}{\ \ \ \ \ \ \ \ \ \ \ \ + 2-layer RQ~\cite{lee2022autoregressive}} & 1: 256 & 11.94 & 89.01 & 0.22 & 0.1595 & 0.5875   \\
& 2: 512 & 6.05 & 113.93 & 0.15  & 0.1547 & 0.5646   \\  \midrule
\multirow{2}{*}{\ \ \ \ \ \ \ \ \ \ \ \ + 2-layer SAQ} & 1: 256 & 12.30 & 93.33 & 0.21 & 0.1613 & 0.5957 \\
& 2: 512 & 5.08 & 125.27 & 0.14  & 0.1595 & 0.5872   \\ \midrule
\multirow{2}{*}{\makecell{\ \ \ \ \ \ \ \ \ \ \ \ + 6-layer pyramid SAQ\\\ \ \ \ \ \ \ \ \ \ \ \ (\cf layer 2-5 in \cref{tab:token_quality})}} & 1: 1 & - & - & - & \textbf{0.1879} & \textbf{0.7196} \\
% & 2: 5 & - & - & - & 0.1868 & 0.7147 \\
% & 3: 21 & - & - & - & 0.1815 & 0.6901 \\
% & 4: 85 & - & - & - & 0.1711 & 0.6414 \\
% & 5: 341 & 9.49 & 109.46 & 0.17 & 0.1604 & 0.5914 \\
& 6: 597 & \textbf{4.41} & \textbf{133.03} & \textbf{0.12}  & 0.1577 & 0.5787   \\ \bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}


==> papers/videopoet/figures/fig_chain_mona_yawn.tex <==
\begin{figure}[ht]
\addtocounter{figure}{-1}
\centering
\begin{subfigure}{0.4\linewidth}
\centering
\videoframe{figures/video_frames/mona_yawn_lores_00001.jpg}
\videoframe{figures/video_frames/mona_yawn_lores_00006.jpg}
\videoframe{figures/video_frames/mona_yawn_lores_00011.jpg}
\videoframe{figures/video_frames/mona_yawn_lores_00017.jpg}
{\textbf{Animated from Still Image}
\ \\
\ \\}
\end{subfigure}
% \vspace{-4mm}


\begin{subfigure}{0.4\linewidth}
\centering
\videoframe{figures/video_frames/mona_yawn_snow_00001.jpg}
\videoframe{figures/video_frames/mona_yawn_snow_00006.jpg}
\videoframe{figures/video_frames/mona_yawn_snow_00011.jpg}
\videoframe{figures/video_frames/mona_yawn_snow_00017.jpg}
{\textbf{Stylized Video} \\
\textbf{Prompt:} An oil painting of a snowman with a red hat opening their mouth to yawn
\ \\}
\end{subfigure}
\captionof{figure}{\textbf{Example of zero-shot video editing via task chaining (text conditioned image-to-video and stylization)} 
%-- the original painting is first animated via a text prompt and then stylized via another text prompt.
}
\label{fig:animate_stylize}
\end{figure}

==> papers/videopoet/figures/fig_chain_train.tex <==
%\begin{figure*}[h]
\begin{figure}[t]
% \addtocounter{figure}{-1} %Prevent subfigures increasing main figure count  % for some reason, this needed to be commented out to get this figure to have a different number than the preceeding figure.
\centering
% Arc shot
\begin{subfigure}[b]{1.0\linewidth}
%{0.5\textwidth}
\centering
\videoframe{figures/video_frames/train_original_00001.jpg}
\videoframe{figures/video_frames/train_original_00006.jpg}
\videoframe{figures/video_frames/train_original_00011.jpg}
\videoframe{figures/video_frames/train_original_00017.jpg}
%\captionof{figure}{Example of directed camera movement }
%\end{figure}
{\textbf{Original Video}
\ \\
\ \\}
\end{subfigure}


\begin{subfigure}[b]{1.0\linewidth}
\centering
\videoframe{figures/video_frames/train_outpaint_00001.jpg}
\videoframe{figures/video_frames/train_outpaint_00006.jpg}
\videoframe{figures/video_frames/train_outpaint_00011.jpg}
\videoframe{figures/video_frames/train_outpaint_00017.jpg}
{\textbf{Outpainted Video}
\ \\
\ \\}
\end{subfigure}


\begin{subfigure}[b]{1.0\linewidth}
\centering
\videoframe{figures/video_frames/train_food_00001.jpg}
\videoframe{figures/video_frames/train_food_00006.jpg}
\videoframe{figures/video_frames/train_food_00011.jpg}
\videoframe{figures/video_frames/train_food_00017.jpg}
{\textbf{Stylized Video} \\
\textbf{Prompt:} A gingerbread and candy train on a track
\ \\}
\end{subfigure}

\caption{\textbf{Example of zero-shot video editing via task chaining (outpainting and stylization)} -- the original video is first outpainted and then stylized via a text prompt.\lu{We can see a clear artifact in the middle row over the train (white block). This image may raise question.}}
\label{fig:outpaint_stylize}
\end{figure}

==> papers/videopoet/figures/fig_inpaint_goat_dragon.tex <==
\begin{figure}[t]
\addtocounter{figure}{-1}

\begin{subfigure}{1.0\linewidth}
\centering
\videoframe{figures/video_frames/goat_original_00001.jpg}
\videoframe{figures/video_frames/goat_original_00006.jpg}
\videoframe{figures/video_frames/goat_original_00011.jpg}
\videoframe{figures/video_frames/goat_original_00017.jpg}
{\textbf{Original Video}
\ \\
\ \\}
\end{subfigure}


\begin{subfigure}{1.0\linewidth}
\centering
\videoframe{figures/video_frames/goat_mask_00001.jpg}
\videoframe{figures/video_frames/goat_mask_00006.jpg}
\videoframe{figures/video_frames/goat_mask_00011.jpg}
\videoframe{figures/video_frames/goat_mask_00017.jpg}
{\textbf{Masked Video}
\ \\
\ \\}
\end{subfigure}


\begin{subfigure}{1.0\linewidth}
\centering
\videoframe{figures/video_frames/goat_dragon_00001.jpg}
\videoframe{figures/video_frames/goat_dragon_00006.jpg}
\videoframe{figures/video_frames/goat_dragon_00011.jpg}
\videoframe{figures/video_frames/goat_dragon_00017.jpg}
{\textbf{Inpainted Video from Text Prompt} \\
\textbf{Prompt:} A blue dragon walking along a ridge
\ \\}
\end{subfigure}

\captionof{figure}{
\textbf{\textbf{Example of a task  the model was not explicitly trained for} -- video editing via text conditioned inpainting.}
}
\label{fig:inpainting_dragon_goat}
\end{figure}

==> papers/videopoet/figures/magvit-v2-config <==
video:
{
  "config": {
    "base_lr": 0.0001,
    "batch_size": "256",
    "data_dtype_str": "float32",
    "dataset_configs": {
      "base_dir": "/readahead/128M",
      "crop_size": "128",
      "dataset_name": "umt_plus_m3",
      "examples_per_subset": {
        "test": "20000",
        "train": "500000000",
        "validation": "20000"
      },
      "frame_rate": "25",
      "label_dir": "/cns/lu-d/home/lijuny/videogvt/datasets",
      "min_resize": "128",
      "num_classes": "0",
      "num_frames": "17",
      "num_test_clips": "1",
      "one_hot_label": false,
      "prefetch_to_device": "2",
      "stride": "1",
      "tables": {
        "test": "/cns/oa-d/home/umt-video-data-access/datasets/umt/25k/raw/e=1:kid=73859:mkey=learning_canon_prod_colossus:mdb=umt-video-data-access/ttl=30d/latest/umt_25k_tokens@100",
        "train": [
          "/cns/vq-d/home/video-first-data-access/canon/umt500m_rgb_noshot_classfiltered/e=1:kid=73859:mkey=learning_canon_prod_colossus:mdb=video-first-data-access/ttl=60d/latest/umt500m_rgb_noshot_classfiltered@20000",
          "/placer/prod/home/viva-video-generation/shutterstock/sstk_ml/e=1:kid=73859:mkey=learning_canon_prod_colossus:mdb=viva-video-generation/latest/sst@99991",
          "/cns/px-d/home/viva-miner/video_miner/faces/rs=6.3/M3/1M/gen/e=1:kid=73859:mkey=learning_canon_prod_colossus:mdb=viva-miner-faces/ttl=30d/latest/viva_miner_faces_m3_1M_train_gen@80000"
        ],
        "validation": "/cns/oa-d/home/umt-video-data-access/datasets/umt/25k/raw/e=1:kid=73859:mkey=learning_canon_prod_colossus:mdb=umt-video-data-access/ttl=30d/latest/umt_25k_tokens@100"
      },
      "train_sample_weights": [
        0.7,
        0.2,
        0.1
      ],
      "train_stride_overrides": [
        "1",
        "1",
        "3"
      ],
      "zero_centering": false
    },
    "dataset_name": "video_sstable_dataset_multitable",
    "discriminator": {
      "channel_multipliers": [
        "2",
        "4",
        "4",
        "4",
        "4"
      ],
      "downsample": "blur",
      "filters": "128",
      "num_remat_blocks": "2"
    },
    "dtype": "float32",
    "eval": {
      "data_splits": "train,test",
      "enable_frechet_distance": true,
      "enable_inception_score": true,
      "enable_lpips": true,
      "enable_ssim_psnr": true,
      "enable_utilization": true,
      "final_num_repeats": "1",
      "num_examples": "20000"
    },
    "eval_batch_size": "64",
    "eval_from": {
      "checkpoint_path": null,
      "step": null,
      "xm": null
    },
    "experiment_name": "UCF101_VQGAN/3D",
    "image_size": "128",
    "init_from": {
      "inflate_discriminator": false,
      "inflation": "2d->3d/last",
      "xm": [
        "64438688",
        "1"
      ]
    },
    "lax_precision": "default",
    "lecam_weight": 0.001,
    "logging": {
      "checkpoint_kept": "5",
      "checkpoint_steps": "1000",
      "enable_checkpoint": true,
      "log_metric_steps": "200",
      "log_sample_size": "2"
    },
    "lr_configs": {
      "base_learning_rate": 0.0001,
      "factors": "constant * cosine_decay * linear_warmup",
      "learning_rate_schedule": "compound",
      "steps_per_cycle": "1000000",
      "warmup_steps": "5000"
    },
    "model_class": "VQGAN",
    "num_training_steps": "1000000",
    "optimizer": {
      "beta1": 0,
      "beta2": 0.99,
      "d_lr": 0.0001,
      "g_lr": 0.0001,
      "lr": 0.0001
    },
    "perceptual_loss_on_logit": true,
    "perceptual_loss_weight": 0.1,
    "polyak_decay": 0.999,
    "pretrained_image_model": true,
    "rng_seed": "0",
    "sq": {
      "bound_method": "sine",
      "dim_widths": [
        "8",
        "8",
        "4",
        "4",
        "4",
        "4",
        "4",
        "4"
      ],
      "quantize_method": "ste"
    },
    "vqgan": {
      "finetune_decoder": false,
      "finetune_path": "",
      "g_adversarial_loss_weight": 0.1,
      "grad_penalty_cost": 10,
      "gradient_penalty": "r1",
      "loss_type": "non-saturating",
      "model_type": "3D"
    },
    "vqvae": {
      "activation_fn": "swish",
      "architecture": "3dcnn",
      "channel_multipliers": [
        "1",
        "2",
        "2",
        "4"
      ],
      "codebook_size": "262144",
      "commitment_cost": 0.25,
      "conv_downsample": true,
      "custom_conv_padding": "causal_custom",
      "decoder_deep_condition": true,
      "deconv_upsample": false,
      "embedding_dim": "8",
      "entropy_loss_ratio": 0.1,
      "entropy_loss_type": "softmax",
      "entropy_temperature": 0.01,
      "filters": "128",
      "norm_type": "GN_spatial",
      "num_dec_remat_blocks": "2",
      "num_dec_res_blocks": "4",
      "num_enc_remat_blocks": "2",
      "num_enc_res_blocks": "4",
      "reconstruction_loss_weight": 5,
      "temporal_downsample": [
        false,
        true,
        true
      ],
      "upsample": "depth_to_space",
      "vector_quantizer_class": "ScalarQuantizer"
    }
  },
  "eval_while_training": "ACTX__MERGE_VALUE_CONFLICT (go/xm-parameters#work-unit-parameters-and-configurations)",
  "logger_levels": null
}
image:
{
  "config": {
    "base_lr": 0.0001,
    "batch_size": "2048",
    "data_dtype_str": "float32",
    "dataset_configs": {
      "dataset": "imagenet2012",
      "gldm_configs": {
        "alt_text_relevance_high_threshold": 0.7,
        "alt_text_relevance_low_threshold": 0.52,
        "drop_dups": true,
        "drop_empty_text": true,
        "ica_labels_score_threshold": 0.95,
        "ica_labels_to_drop_by": null,
        "ignore_errors": true,
        "max_ica_labels": "3",
        "prefer_alt_text_prob": 1,
        "prepend_ica_labels_prob": 1,
        "random_pali_caption": true,
        "use_proxy": false
      },
      "gldm_ds_names": {
        "train": "webli_v3_tigg_data_v1"
      },
      "image_size": "128",
      "num_classes": "0",
      "pp_eval": "decode|resize_small(128)|central_crop(128)|value_range(0, 1)|copy(\"label\", \"labels\")|keep(\"image\", \"labels\")",
      "pp_train": "keep(\"image\")",
      "prefetch_to_device": "2",
      "shuffle_buffer_size": "10000",
      "text_encoder_name": "dummy",
      "train_split": "train",
      "val_split": "validation"
    },
    "dataset_name": "webli",
    "dataset_type": "image",
    "discriminator": {
      "blur_resample": true,
      "channel_multipliers": [
        "2",
        "4",
        "4",
        "4",
        "4"
      ],
      "filters": "128"
    },
    "dtype": "float32",
    "eval": {
      "data_splits": "train,validation",
      "enable_frechet_distance": false,
      "enable_frechet_image_distance": true,
      "enable_inception_score": false,
      "enable_lpips": true,
      "enable_ssim_psnr": true,
      "enable_utilization": true,
      "final_num_example_multiplier": "5",
      "num_examples": "10000"
    },
    "eval_batch_size": "64",
    "eval_dataset_name": "bit",
    "eval_from": {
      "checkpoint_path": null,
      "step": null,
      "xm": null
    },
    "experiment_name": "ImageNet_VQGAN/2D",
    "image_size": "128",
    "lax_precision": "default",
    "lecam_weight": 0.001,
    "logging": {
      "checkpoint_kept": "5",
      "checkpoint_steps": "10000",
      "enable_checkpoint": true,
      "log_metric_steps": "200",
      "log_sample_size": "8"
    },
    "lr_configs": {
      "base_learning_rate": 0.0001,
      "factors": "constant * cosine_decay * linear_warmup",
      "learning_rate_schedule": "compound",
      "steps_per_cycle": "1000000",
      "warmup_steps": "10000"
    },
    "model_class": "VQGAN",
    "num_training_steps": "1000000",
    "optimizer": {
      "beta1": 0,
      "beta2": 0.99,
      "d_lr": 0.0001,
      "g_lr": 0.0001,
      "lr": 0.0001
    },
    "perceptual_loss_on_logit": true,
    "perceptual_loss_weight": 0.1,
    "polyak_decay": 0.999,
    "pretrained_image_model": true,
    "rng_seed": "0",
    "sq": {
      "bound_method": "sine",
      "dim_widths": [
        "8",
        "8",
        "4",
        "4",
        "4",
        "4",
        "4",
        "4"
      ],
      "quantize_method": "ste"
    },
    "vqgan": {
      "g_adversarial_loss_weight": 0.1,
      "grad_penalty_cost": 10,
      "gradient_penalty": "r1",
      "loss_type": "non-saturating",
      "model_type": "2D"
    },
    "vqvae": {
      "activation_fn": "swish",
      "architecture": "2dcnn",
      "channel_multipliers": [
        "1",
        "2",
        "2",
        "4"
      ],
      "codebook_size": "262144",
      "commitment_cost": 0.25,
      "conv_downsample": true,
      "decoder_deep_condition": true,
      "deconv_upsample": false,
      "embedding_dim": "8",
      "entropy_loss_ratio": 0.1,
      "entropy_loss_type": "softmax",
      "entropy_temperature": 0.01,
      "filters": "128",
      "norm_type": "GN",
      "num_attn_heads": "8",
      "num_dec_res_blocks": "4",
      "num_enc_res_blocks": "4",
      "reconstruction_loss_weight": 5,
      "upsample": "depth_to_space",
      "use_attn": false,
      "vector_quantizer_class": "ScalarQuantizer"
    }
  },
  "eval_while_training": "ACTX__MERGE_VALUE_CONFLICT (go/xm-parameters#work-unit-parameters-and-configurations)",
  "logger_levels": null
}


==> papers/videopoet/figures/video_samples.tex <==
\begin{figure*}%[!hb]
\begin{subfigure}{0.5\textwidth}
\centering
\videoframe{figures/video_frames/00335_.cfg_4.0.temp_1.0.topp_0.95_a_photorealistic_teddy_bear_is_holding_hands_sr_bins_24_temp_14.5.mp4_001.png}
\videoframe{figures/video_frames/00335_.cfg_4.0.temp_1.0.topp_0.95_a_photorealistic_teddy_bear_is_holding_hands_sr_bins_24_temp_14.5.mp4_003.png}
\videoframe{figures/video_frames/00335_.cfg_4.0.temp_1.0.topp_0.95_a_photorealistic_teddy_bear_is_holding_hands_sr_bins_24_temp_14.5.mp4_004.png}
\videoframe{figures/video_frames/00335_.cfg_4.0.temp_1.0.topp_0.95_a_photorealistic_teddy_bear_is_holding_hands_sr_bins_24_temp_14.5.mp4_006.png}
{\textbf{ Prompt}: A photorealistic teddy bear is holding hands with another teddy bear, walking down 5th avenue when it is raining
\ \\
\ \\}
\end{subfigure}
~
\begin{subfigure}{0.5\textwidth}
\centering
\videoframe{figures/video_frames/mane_00001.jpg}
\videoframe{figures/video_frames/mane_00025.jpg}
\videoframe{figures/video_frames/mane_00030.jpg}
\videoframe{figures/video_frames/mane_00037.jpg}\\
{\textbf{ Prompt}: A lion with a mane made out of yellow dandelion petals roars
\ \\
\ \\
\ \\}
\end{subfigure}
~
\begin{subfigure}{0.5\textwidth}
\centering
\videoframe{figures/video_frames/00104_cfg_3.2.temp_1.0.topp_0.95_a_dog_listening_to_music_with_headphones,_highly_detailed,_cinematic,_high_contrast,_8k_3.gif_001.png}
\videoframe{figures/video_frames/00104_cfg_3.2.temp_1.0.topp_0.95_a_dog_listening_to_music_with_headphones,_highly_detailed,_cinematic,_high_contrast,_8k_3.gif_003.png}
\videoframe{figures/video_frames/00104_cfg_3.2.temp_1.0.topp_0.95_a_dog_listening_to_music_with_headphones,_highly_detailed,_cinematic,_high_contrast,_8k_3.gif_005.png}
\videoframe{figures/video_frames/00104_cfg_3.2.temp_1.0.topp_0.95_a_dog_listening_to_music_with_headphones,_highly_detailed,_cinematic,_high_contrast,_8k_3.gif_006.png}
{\textbf{ Prompt}:  A dog listening to music with headphones, highly detailed, 8k
\ \\
\ \\}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\centering
\videoframe{figures/video_frames/chicken_00001.jpg}
\videoframe{figures/video_frames/chicken_00005.jpg}
\videoframe{figures/video_frames/chicken_00009.jpg}
\videoframe{figures/video_frames/chicken_00012.jpg}
{\textbf{ Prompt}: A chicken lifting weights
\ \\
\ \\
\ \\}
\end{subfigure}

\begin{subfigure}{1.0\textwidth}
\centering
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00001.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00004.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00008.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00012.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00017.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00023.jpg}
%\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00033.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00038.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00049.jpg}
{\textbf{ Prompt}: A large blob of exploding splashing rainbow paint, with an apple emerging, 8k
\ \\}
\end{subfigure}
\caption{\textbf{Examples from \modelname{}'s text-to-video generation
results.} Some prompts are edited for clarity.}
\label{fig:video_samples}
\end{figure*}

